Strong Faithfulness for ELH Ontology Embeddings

Ontology embedding methods are powerful approaches to represent and reason over structured knowledge in various domains. One advantage of ontology embeddings over knowledge graph embeddings is their ability to capture and impose an underlying schema to which the model must conform. Despite advances, most current approaches do not guarantee that the resulting embedding respects the axioms the ontology entails. In this work, we formally prove that normalized ${\cal ELH}$ has the strong faithfulness property on convex geometric models, which means that there is an embedding that precisely captures the original ontology. We present a region-based geometric model for embedding normalized ${\cal ELH}$ ontologies into a continuous vector space. To prove strong faithfulness, our construction takes advantage of the fact that normalized ${\cal ELH}$ has a finite canonical model. We first prove the statement assuming (possibly) non-convex regions, allowing us to keep the required dimensions low. Then, we impose convexity on the regions and show the property still holds. Finally, we consider reasoning tasks on geometric models and analyze the complexity in the class of convex geometric models used for proving strong faithfulness.

==> complexity.tex <==
%In this \lcnamecref{sec:modelcheck}, 
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetAlgoLined
    \LinesNumbered
    \caption{Check if a convex geometric model (\cref{def:geoconvex}) satisfies an \ELH CI in normal form}
    \label{alg:conceptsubalgo}
    
    \SetKwProg{Fn}{Function}{:}{end}
    \SetKw{null}{null}
    
    \SetArgSty{textnormal}
    
    \KwIn{A convex geometric interpretation \(\geoconvex\) and an \ELH concept inclusion in normal form \(\alpha\)}
    \KwOut{\valtrue if \(\geoconvex \models \alpha\), \valfalse otherwise}
    \tcp*[l]{\(A, A_1, A_2, B \in \NC \cup \{\top\}\), \(r \in \NR\)}
    \If{\(\alpha = A \sqsubseteq B\)}{
        \lIf{\(B = \top\)}{\nllabel{CInf1start}
            \Return{\valtrue}
        }
        \For{\(v \in \geointerp(A)\)}{\nllabel{CInf1loopstart}
            \lIf{\(v[B] = 0\)}{\nllabel{CInf1check}
                \Return{\valfalse}\nllabel{CInf1loopend}\nllabel{CInf1end}
            } 
        }
    }
    \ElseIf{\(\alpha = A_1 \sqcap A_2 \sqsubseteq B\)}{
        \lIf{\(B = \top\)}{\nllabel{CInf2start}
            \Return{\valtrue}
        }
        \For{\(v \in \geointerp(A_1)\)}{\nllabel{CInf2loopstart}
            \If{\((A_2 = \top \lor v[A_2] = 1) \land v[B] = 0\)}{\nllabel{CInf2check}
                \Return{\valfalse}\nllabel{CInf2end}
            } 
        }
    }
    \ElseIf{\(\alpha = A \sqsubseteq \exists r.B\)}{
        \For{\(v \in \geointerp(A)\)}{\nllabel{CInf3loopstart}
            count \(\gets\) 0\; 
            \For{\(u \in \geointerp(B)\)}{
                \If{\(v \oplus u \in \geointerp(r)\)}{\nllabel{CInf3lookup}
                    count \(\gets\) count + 1\; 
                }
            }\nllabel{CInf3loopend}
            \lIf{count = 0}{
                \Return{\valfalse}
            }
        }
    }
    \ElseIf{\(\alpha = \exists r.A \sqsubseteq B\)}{
        \lIf{\(B = \top\)}{\nllabel{CInf4start}
            \Return{\valtrue}
        }
        \For{\(v \oplus u \in \geointerp(r)\)}{\nllabel{CInf4loopstart}
            \If{\(u[A] = 1\) and \(v[B] = 0\)}{
                \Return{\valfalse}\nllabel{CInf4end}
            }
        }
    }
    \Return{\valtrue}
\end{algorithm}

Here we study upper bounds for the complexity of model checking problems using convex geometric models  as those defined  in \cref{def:geoconvex} and normalized \(\ELH\) axioms.
The results and algorithms in this section are underpinned by \cref{aggregatedlemma}, which allow us to use \(\geointerp\) instead of \(\geoconvex\) for model checking purposes. 
The advantage of using \(\geointerp\) instead of \(\geoconvex\) is that the algorithms need to inspect only finitely many elements in the extension of each concept and each role, as long as the original interpretation \(\I\) has finite domain (and we only need to consider a finite number of concept, role, and individual names).
For example, let \(\I = (\Delta^\I, \cdot^\I)\) with \(\Delta^\I\) finite.
If \(A \in \NC\) then \(\geoconvex(A)\) can have infinitely many elements, while \(\geointerp(A)\)  will have at most \(\sizedelta\) elements (by \cref{def:geointerp2}).

Before presenting the algorithms, we discuss some assumptions that   facilitate our analysis:
\begin{enumerate}
    \item\label{assumptionBasic} indexing vectors and comparing primitive types use constant time;
    \item\label{assumptionAccess} accessing the extension of an individual name, concept name, or role name in \(\geointerp\) takes constant time;
    \item\label{assumptionIter} iterating over \(\geointerp(A)\) (\(\geointerp(r)\)) consumes time \(O(\sizedelta)\) (\(O(\sizedeltas)\)) for all \(A \in \NC\) (\(r \in \NR\)); and
    \item\label{assumptionMember} if \(A \in \NC\) (\(r \in \NR\)), testing if \(v \in \geointerp(A)\) (\(v \in \geointerp(r))\) consumes time \(O(\dimsymb \cdot \sizedelta)\) (\(O(\dimsymb \cdot \sizedeltas)\)).
\end{enumerate}

Assumption (1) is standard when analysing worst-case complexity.
The others are pessimistic assumptions on the implementation of \(\geointerp\) (and \(\geoconvex\)).
E.g., encoding the binary vectors as integers and implementing bit wise operations could reduce the complexity of membership access and iteration.
Also, using a hash map with a perfect hash function would decrease the membership check to constant time.


%\Cref{hull_before_after} provides the main result that facilitates the design of said \lcnamecref{alg:conceptsubalgo}.

%\begin{lemma}%
%\label{hull_before_after}\todo{Useless here given \cref{tboxnonconvex,lem:tboxconvex}}
%    Let \(C\) be an \ELH concept in normal form and \(\geointerp\) a geometric interpretation.
%    Then \({(\geointerp(C))}^* = \geoconvex(C)\).
%    \todo{Do we need to specify that \(C\) is in the signature of \(\I\)?}
%\end{lemma}
%
%\begin{proof}
%    We divide the proof in cases. In all of them \(A, B \in \NC \cup \{\top\}\).
%    \begin{description}
%        \item[\(C = A\):] In this case, the \lcnamecref{hull_before_after} follows directly from the definition of \(\geoconvex\) (\cref{def:geoconvex}). 
%        %
%        \item[\(C = A \sqcap B\):] By the semantics of \ELH, we get from the definition of \(\geointerp\) (\cref{def:geointerp2}) that \(\geointerp(A \sqcap B) = \geointerp(A) \cap \geointerp(B)\) and from \cref{def:geoconvex} that \(\geoconvex(A \sqcap B) = \geoconvex(A) \cap \geoconvex(B)\).
%        From the previous item, \({(\geointerp(A))}^* = \geoconvex(A)\) and \({(\geointerp(B))}^* = \geoconvex(B)\).
%        Hence, \(\geoconvex(A \sqcap B) = {(\geointerp(A))}^* \cap {(\geointerp(B))}^*\).
%        We will show next that \({(\geointerp(A) \cap \geointerp(B))}^* = {(\geointerp(A))}^* \cap {(\geointerp(B))}^*\).
%        First, let \(v \in {(\geointerp(A) \cap \geointerp(B))}^*\).
%        By definition of convex hull (\cref{defconvexhull}), there are \(0 \leq \lambda_1, \dots, \lambda_n \leq 1\) with \(\sum_{i = 1}^n \lambda_i = 1\) and \(v_i \in ((\geointerp(A) \cap \geointerp(B))\) such that \(v = \sum_{i=1}^n \lambda_i v_i\).
%        As \(v_i \in \geointerp(A)\) and \(v_i \in \geointerp(B)\), for \(1 \leq i \leq n\), we also get that \(v \in \geointerp(A)^*\) and \(v \in \geointerp(B)^*\).
%        Therefore, \({(\geointerp(A) \cap \geointerp(B))}^* \subseteq {(\geointerp(A))}^* \cap {(\geointerp(B))}^*\).
%        Now, let  \(v' \in {(\geointerp(A))}^* \cap {(\geointerp(B))}^*\).
%        By \cref{defconvexhull}, there are \(0 \leq \lambda'_1, \dots, \lambda'_m \leq 1\) with \(\sum_{i = 1}^m \lambda'_j = 1\) and \(v'_j \in \geointerp(A)\) such that \(v' = \sum_{j=1}^m \lambda'_j v'_j\).
%        We get from \cref{def:geointerp2} that \(v[B] = 1\), as \(0 \leq \lambda'_1, \dots, \lambda'_m \leq 1\) and \(\sum_{i = 1}^m \lambda'_j = 1\) it must be the case that \(v'_j[B] = 1\).
%        \todo{Very similar to a step in the proof of \cref{reminderanchor} item (3)}
%        This implies that \(v'_j \in \geointerp(A) \cap \geointerp(B)\), from which can conclude that \(v' \in {(\geointerp(A) \cap \geointerp(B))}^*\).
%        Therefore, \({(\geointerp(A))}^* \cap {(\geointerp(B))}^* \subseteq {(\geointerp(A) \cap \geointerp(B))}^*\).
%        We can finally conclude that  \({(\geointerp(A) \cap \geointerp(B))}^* = {(\geointerp(A))}^* \cap {(\geointerp(B))}^*\).
%        In other words, \({(\geointerp(A \sqcap B))}^* = \geoconvex(A \sqcap B)\).
%        %
%        \item[\(C = \exists r.A\):] Let \(v \in {(\geointerp(\exists r.A))}^*\).
%        By \cref{defconvexhull}, there are \(0 \leq \lambda_1, \dots, \lambda_n \leq 1\) with \(\sum_{i = 1}^n \lambda_i = 1\) and \(v_i \in \geointerp(\exists r.A)\) such that \(v = \sum_{i=1}^n \lambda_i v_i\).
%        Thus, by the semantics of \ELH, for each \(v_i\) there is an \(u_i \in \geointerp(A)\) with \(v_i \oplus u_i \in \geointerp(r)\).
%        By \cref{convexsubsetobvious}, \(v_i \oplus u_i \in \geoconvex(r)\) and \(u_i \in \geoconvex(A)\).
%        We obtain \(v_i \in \geoconvex(\exists r.A)\) from \cref{def:geoconvex}, and hence, we can conclude \({(\geointerp(\exists r.A))}^* \subseteq \geoconvex(\exists r.A)\).
%        Now, let \(v' \in \geoconvex(\exists r.A)\).
%        By \cref{def:geoconvex}, there is an \(u' \in \geoconvex(A)\) such that \(v' \oplus u' \in \geoconvex(r)\).
%        As a consequence of \cref{defconvexhull}, there are \(v_1, \dots, v_m, u_1, \dots, u_m \in \Rdim\) and \(0 \leq \lambda'_1, \dots, \lambda'_m \leq 1\) such that \(\sum_{i = 1}^m \lambda'_j = 1\), \(v'_j \oplus u'_j \in \geointerp(r)\) and \(v' \oplus u' = \sum_{j=1}^m \lambda'_j (v'_j \oplus u'_j)\).
%        From \cref{Lemma: v in eta estrela A}, we get \(u'[A] = 1\), thus, \(u'_j[A] = 1\) since \(0 \leq \lambda'_1, \dots, \lambda'_m \leq 1\) and \(\sum_{i = 1}^m \lambda'_j = 1\).
%        \todo{Again, very similar to a step in the proof of \cref{reminderanchor} item (3).}
%        Moreover, \cref{vinetarimpliesvmud2} implies that for every \(1 \leq j \leq m\), there is an \(e_j \in \Delta^\I\) with \(\mu(e_j) = u'_j\).
%        As we proved that \(u'_j[A] = 1\), it follows from \cref{def:geointerp2} that \(u'_j \in \geointerp(A)\).
%        Hence, we have \(v'_j \in \geointerp(\exists r.A)\) for all \(1 \leq j \leq m\).
%        Since \(v' \oplus u' = \sum_{j=1}^m \lambda'_j (v'_j \oplus u'_j)\), it holds that \(\sum_{j=1}^m \lambda'_j v'_j = v'\).
%        In other words, \(v' \in {(\geointerp(\exists r.A))}^*\) and we obtain \(\geoconvex(\exists r.A) \subseteq {(\geointerp(\exists r.A))}^*\).
%        Thus, \(\geoconvex(\exists r.A) = {(\geointerp(\exists r.A))}^*\).
%        \qedhere
%    \end{description}
%\end{proof}


%\Cref{aggregatedlemma} ensures that it is sufficient to consider elements in \(\geointerp(A)\) for all \(A \in \NC\) and pairs in \(\geointerp(r)\) for all \(r \in \NR\) when deciding whether \(\geoconvex\) models an \ELH concept inclusion in normal form.
We are now ready to present our upper bounds. For normalised \ELH CIs, we provide \cref{alg:conceptsubalgo} to decide if a concept inclusion holds in a convex geometric model built as in \cref{def:geoconvex}.
\Cref{aggregatedlemma} guarantees that \(\geoconvex \models C \sqsubseteq D\) iff \(\geointerp \models C \sqsubseteq D\) for any CI in normalised \ELH.
Thus, as long as \(\Delta^\I\) is finite, \cref{alg:conceptsubalgo} terminates and outputs whether \(\geoconvex \models C \sqsubseteq D\).
\Cref{conceptsub_complexity} establishes that \cref{alg:conceptsubalgo} runs in 
polynomial time in the size of \(\Delta^\I\) and the dimension of  vectors in \(\geoconvex\).
%Additionally, if set membership (lookup) takes only constant time (e.g.\ via a hash map with perfect hash), then the algorithm consumes time linear in \(|\Delta^\I|\).

\begin{restatable}{theorem}{algoplexityconceptinclusion}
\label{conceptsub_complexity}
    Given a finite geometric interpretation \(\geointerp\) and an \ELH CI in normal form,
    \cref{alg:conceptsubalgo} runs in time in \(O(\dimsymb \cdot \sizedeltaabbrev^4)\), where \(\dimsymb\) is as in \cref{mu2definition} and \(\sizedeltaabbrev = |\Delta^\I|\).
\end{restatable}

%\begin{proof}
%    \Cref{alg:conceptsubalgo} has four main parts that are never executed in the same run, each corresponding to one of the normal forms that the input concept inclusion \(\alpha\) can take.

%    \begin{description}
%        \item[\(\alpha = A \sqsubseteq B\):] In this case, the algorithm will execute lines \crefrange{CInf1start}{CInf1end}.
%        From assumption~\ref{assumptionBasic}, \cref{CInf1check} spends time \(O(1)\) and by assumption~\ref{assumptionIter} this line is run \(O(\sizedelta)\) times. 
%        Hence, in this case, the algorithm consumes time \(O(\sizedelta)\).

%        \item[\(\alpha = A_1 \sqcap A_2 \sqsubseteq B\):] From assumption~\ref{assumptionIter}, the loop from \crefrange{CInf2loopstart}{CInf2end} is executed \(O(\sizedelta)\) times.
%        Each iteration consumes time \(O(1)\) by assumption~\ref{assumptionBasic}. 
%        Thus, \cref{alg:conceptsubalgo} runs in time \(O(\sizedelta)\) in this case.

%        \item[\(\alpha = A \sqsubseteq \exists r.B\):] 
%        According to assumption~\ref{assumptionIter}, the nested loop from \crefrange{CInf3loopstart}{CInf3loopend} uses time \(O(\sizedeltas)\).
%        The membership check in \cref{CInf3lookup} takes time \(O(\dimsymb \cdot \sizedeltas)\), by assumption~\ref{assumptionMember}.
%        Therefore, we get that \cref{alg:conceptsubalgo} requires time \(O(\dimsymb \cdot \sizedeltaabbrev^4)\), where \(\sizedeltaabbrev = \sizedelta\).

%        \item[\(\alpha = \exists r.A \sqsubseteq B\):] \Cref{alg:conceptsubalgo} will execute from \crefrange{CInf4start}{CInf4end} for CIs in this normal form.
%        Each iteration of the for loop starting in \cref{CInf4loopstart} consumes constant time according to assumption~\ref{assumptionBasic}.
%        Furthermore, the loop has \(O(\sizedeltas)\) iterations due to assumption~\ref{assumptionIter}.
%        Hence, \cref{alg:conceptsubalgo} uses time \(O(\sizedeltas)\) for CIs in this normal form.
%    \end{description}
%    Therefore, \cref{alg:conceptsubalgo} consumes time \(O(\dimsymb \cdot \sizedeltaabbrev^4)\).
%\end{proof}

As \(\dimsymb\) depends linearly on \(\Delta^\I\) and the size of the signature.
If the latter is regarded as a constant, we can simply say that \cref{alg:conceptsubalgo} has time in \(O(\sizedeltaabbrev^5)\), where \(\sizedeltaabbrev = \sizedelta\).
Similarly as for \cref{alg:conceptsubalgo}, \cref{aggregatedlemma} allows us to design an algorithm to determine if a convex geometric model \(\geoconvex\) satisfies an IQ in normal form \(\alpha\), as we show in \cref{alg:IQs}.
%\begin{algorithm}[tbph]
%    \DontPrintSemicolon
%    \SetAlgoLined
%    \LinesNumbered
%    \caption{Deciding instance queries with our convex geometric model}
%    \label{alg:conceptIQ}
%    
%    \SetKwProg{Fn}{Function}{:}{end}
%    \SetKw{null}{null}
%    \SetKwFunction{FExt}{Ext}
%    \SetKwFunction{FBelongs}{checkConceptAssertion}
%    
%    \KwIn{A geometric interpretation \(\geointerp\) and an \ELH concept assertion \(C(a)\)}
%    \KwOut{\valtrue if \(\geoconvex \models \alpha\), \valfalse otherwise}
%
%    \Fn{\FExt{\(C\)}}{\nllabel{extensionFnStart}\nllabel{extfn}
%        \If{\(C \in \NC \cup \{\top\}\)}{\nllabel{extbasecasestart}
%            \Return{\(\geointerp(C)\)}\nllabel{extbasecaseend}
%        }
%        \ElseIf{\(C = C_1 \sqcap C_2\)}{
%            \Return{\FExt{\(C_1\)} \(\cap\) \FExt{\(C_2\)}}\nllabel{extConj}
%        }
%        \ElseIf{\(C = \exists r.C'\)}{\nllabel{extExistStart}
%            S \(\gets \emptyset\)\;
%            \For{\(v \oplus u \in \geointerp(r)\)}{\nllabel{extExistLoopStart}
%                \If{\(u \in\)\FExt{\(C'\)}}{\nllabel{extExistRec}
%                    \If{\(v \oplus u \in \geointerp(r)\)}{\nllabel{extExistMemberCheck}
%                        S \(\gets\) S \(\cup \{v\}\)\;
%                    }
%                }
%            }
%            \Return{S}\nllabel{extExistEnd}
%        }
%    }
%
%    \Fn{\FBelongs{\(C(a)\)}}{
%        \Return{\(\geointerp(a) \in\) \FExt{\(C\)}}\nllabel{membershipCheck}
%    }
%\end{algorithm}
%\begin{theorem}%
%\label{conceptIQcomplexity}
%    If deciding membership of vectors in extensions by \(\geointerp\) takes polynomial time in \(|\Delta^\I|\), then
%    \Cref{alg:conceptIQ} runs in polynomial time in \(\lengthCon(C) \cdot |\Delta^\I|\) where \(\lengthCon(C)\) is defined as
%    \begin{align*}
%        \lengthCon(C) =
%        \begin{cases}
%            1 &\text{if } C \in \NC \cup \{\top\}\\
%            \lengthCon(C_1) + \lengthCon(C_2) + 1 &\text{if } C = C_1 \sqcap C_2\\
%            \lengthCon(C') + 1 &\text{if } C = \exists r.C'.
%        \end{cases}
%    \end{align*}
%    %Also, if deciding membership of vectors in extensions by \(\geointerp\) takes constant time, then \cref{alg:conceptsubalgo} runs in time \(O(\lengthCon(C) \cdot (|\Delta^\I \times \Delta^\I|))\).
%\end{theorem}
%\begin{proof}
%    The proof follows by induction in the structure of the concept \(C\) of an arbitrary input \ELH concept assertion \(C(a)\).
%
%    \paragraph{Base:} In the base case, \(C \in \NC \cup \{\top\}\), hence, \(\lengthCon(C) = 1\).
%    This means that the algorithm will perform a single call to \FExt, which will return \(\geointerp(C)\) in constant time.
%    Thus, if we assume that \cref{membershipCheck} consumes time polynomial in \(|\Delta^\I|\), \cref{alg:conceptIQ} will also run in time polynomial in \(|\Delta^\I|\).
%    Furthermore, if we assume that \cref{membershipCheck} takes constant time, then the algorithm runs in time \(O(|\Delta^\I|)\) for this input.
%
%    \paragraph{Induction Step:} Assume that our hypothesis holds for the concepts \(C_1\) and \(C_2\).
%    We consider two cases.
%
%    \begin{description}
%        \item[\(C = C_1 \sqcap C_2\):] In this case, \cref{alg:conceptIQ} executes \cref{extConj}.
%        By our induction hypothesis, computing \FExt(\(C_i\)) takes time polynomial %(quadratic if membership takes only constant time) 
%        time in \(\lengthCon(C_i) \cdot |\Delta^\I|\).
%        Hence, \cref{extConj} will take the time spent by each call to \FExt and additional time to perform the intersection, which can also be performed in polynomial time in \(\lengthCon(C_i) \cdot |\Delta^\I|\).% (linear if membership checks take constant time).
%        Thus, in this case, \FExt{\(C\)} consumes time polynomial in \((\lengthCon(C_1) + \lengthCon(C_2) + 1) \cdot |\Delta^\I|\).
%        Therefore, as we assume that \cref{membershipCheck} consumes time polynomial in \(|\Delta^\I|\), we have that \cref{alg:conceptIQ} consumes polynomial time in \(\lengthCon(C) \cdot |\Delta^\I|\).
%
%        \item[\(C = \exists r.C_1\):] For concepts of this form, the call \FExt{\(C\)} will run lines \crefrange{extExistStart}{extExistEnd}.
%        We know from \cref{def:geointerp2} that \(|\geointerp(\top) = |\Delta^\I|\), therefore, the loop declared in \cref{extExistLoopStart} will run at most \(|\Delta^\I|\) times.
%        The call to \FExt in \cref{extExistRec} will consume time polynomial in \(\lengthCon(C') \cdot |\Delta^\I|\) by the induction hypothesis.
%        Additionally, we assume that the operations in \crefrange{extExistMemberCheck}{extExistEnd} each takes polynomial time in \(|\Delta^\I|\).
%        Therefore, as we assume that \cref{membershipCheck} consumes time polynomial in \(|\Delta^\I|\), we have that \cref{alg:conceptIQ} consumes polynomial time in \(\lengthCon(C) \cdot |\Delta^\I|\).
%    \end{description}
%
%    Thus, we have proved that for every \ELH concept assertion \cref{alg:conceptIQ} runs in time polynomial on \(\lengthCon(C)\) 
%\end{proof}
%Role assertions and role inclusions are significantly simpler to decide using convex geometric models.
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetAlgoLined
    \LinesNumbered
    
    \caption{Check if a convex geometric model (as in \cref{def:geoconvex}) satisfies an \ELH IQ in normal form}
    \label{alg:IQs}
    
    \SetKwProg{Fn}{Function}{:}{end}
    \SetKw{null}{null}
    \SetArgSty{textnormal}
    
    \KwIn{A convex geometric interpretation \(\geoconvex\) and an \ELH IQ in normal form \(\alpha\)}
    \KwOut{\valtrue if \(\geoconvex \models \alpha\), \valfalse otherwise}

    
    \tcp*[l]{\(A, B \in \NC \cup \{\top\}\), \(r \in \NR\), \(a, b \in \NI\)}
    \If{\(\alpha = A(a)\)}{
        \lIf{\(A = \top \lor \geointerp(a)[A] = 1\)}{\nllabel{IQnf1check}
            \Return{\valtrue}
        }
    }
    \ElseIf{\(\alpha = (A \sqcap B)(a)\)}{
        \If{\((A = \top \lor \geointerp(a)[A] = 1) \land (B = \top \lor \geointerp(a)[B] = 1)\)}{\nllabel{IQnf2check}
            \Return{\valtrue}
        }
    }
    \ElseIf{\(\alpha = (\exists r.A)(a)\)}{
        \For{\(u \in \geointerp(A)\)}{\nllabel{IQ3loopstart}
            \If{\(\geointerp(a) \oplus u \in \geointerp(r)\)}{\nllabel{IQnf3lookup}
                \Return{\valtrue}\; 
            }
        }\nllabel{IQnf3loopend}
    }
    \ElseIf{\(\alpha = r(a, b)\)}{
        \If{\(\geointerp(a) \oplus \geointerp(b) \in \geointerp(r)\)}{\nllabel{IQnf4check}
            \Return{\valtrue}
        }
    }
    \Return{\valfalse}
\end{algorithm}

\Cref{normIQ_complexity} shows that \cref{alg:IQs} %the complexity of model checking with convex geometric models for \ELH IQs in normal form is also 
runs in time polynomial in \(\dimsymb \cdot \sizedelta\).

\begin{restatable}{theorem}{algoplexitynormIQ}%
\label{normIQ_complexity}
    Given a finite geometric interpretation \(\geointerp\) and an \ELH IQ in normal form,
    \cref{alg:IQs} runs in time \(O(\dimsymb \cdot \sizedeltaabbrev^3)\), with \(\dimsymb\)  as in \cref{mu2definition} and \(\sizedeltaabbrev = |\Delta^\I|\).
\end{restatable}

%\begin{proof}
%    We consider each the four forms that an \ELH IQ in normal form \(\alpha\) can assume separately.
%    In each of them \(a \in \NI\), \(A, B \in \NC\), and \(r \in \NR\).

%    \begin{description}
%        \item[\(\alpha = A(a)\):] Due to assumptions~\ref{assumptionBasic} and~\ref{assumptionAccess}, \cref{IQnf1check} uses time \(O(1)\).
%        \item[\(\alpha = (A \sqcap B)(a)\):] As in the previous case, the assumption~\ref{assumptionBasic} and~\ref{assumptionBasic} imply that \cref{IQnf2check} executes in time \(O(1)\).
%        \item[\(\alpha = (\exists r.A)(a)\):] By assumption~\ref{assumptionIter}, \cref{IQnf3lookup} is run \(O(\sizedelta)\) times, each iteration consuming time in \(O(\dimsymb \cdot \sizedeltas)\) (from assumptions~\ref{assumptionAccess} and~\ref{assumptionMember}).
%        Therefore, \cref{alg:IQs} spends time \(O(\dimsymb \cdot \sizedeltaabbrev^3)\) in such instance queries, where \(\sizedeltaabbrev = \sizedelta\).
%        \item[\(\alpha = r(a, b)\):] \Cref{IQnf4check} runs in time \(O(\dimsymb \cdot \sizedeltas)\) due to assumptions~\cref{assumptionAccess} and~\ref{assumptionMember}.
%    \end{description}
    
%    Therefore, \cref{alg:IQs} consumes time \(O(\dimsymb \cdot \sizedeltaabbrev^3)\).
%\end{proof}

Next, we present \cref{alg:RIs}, which handles RIs.
Again, as a consequence of \cref{aggregatedlemma}, we only need to check the inclusion between two finite sets of vectors in \(\mathbb{R}^{2 \cdot \dimsymb}\).

\begin{algorithm}[tbph]
        \DontPrintSemicolon
    \SetAlgoLined
    \LinesNumbered
    
    \caption{Check if a convex geometric model (as in \cref{def:geoconvex}) satisfies an \ELH role inclusion}
    \label{alg:RIs}
    
    \SetKwProg{Fn}{Function}{:}{end}
    \SetKw{null}{null}
    
    \SetArgSty{textnormal}
    
    \KwIn{A convex geometric interpretation \(\geoconvex\) and an \ELH role inclusion \(r \sqsubseteq s\)}
    \KwOut{\valtrue if \(\geoconvex \models r \sqsubseteq s\), \valfalse otherwise}

    \tcp*[l]{\(r,s \in \NR\)}
    \For{\(v \in \geointerp(r)\)}{\nllabel{RIloop}
        \If{\(v \not \in \geointerp(s)\)}{\nllabel{RIcheck}
            \Return{\valfalse}
        }
    }
    \Return{\valtrue}
\end{algorithm}

Finally, we show an upper bound using \cref{alg:RIs}.

\begin{restatable}{theorem}{algoplexitynormRI}%
\label{normRI_complexity}
    Given a finite geometric interpretation \(\geointerp\) and an \ELH role inclusion,
    \cref{alg:RIs} runs in time in \(O(\dimsymb \cdot \sizedeltaabbrev^4)\), where \(\dimsymb\) is as in \cref{mu2definition} and \(\sizedeltaabbrev = |\Delta^\I|\).
\end{restatable}

%\begin{proof}
%    There are \(O(\sizedeltas)\) iterations of the for loop starting in \cref{RIloop} in a single run of \cref{alg:RIs} as a consequence of the assumptions~\ref{assumptionIter}.
%    Additionally, each iteration consumes time \(O(\dimsymb \cdot \sizedeltas)\) by assumption~\ref{assumptionMember}.
%    Therefore, \cref{alg:RIs} runs in time \(O(\dimsymb \cdot \sizedeltaabbrev^4)\), where \(\sizedeltaabbrev = \sizedelta\).
%\end{proof}

The three algorithms presented in this \lcnamecref{sec:modelcheck} run in polynomial time in \(\dimsymb \cdot \sizedelta\).
We recall that the construction of \(\geointerp\) (and by extension of \(\geoconvex\)) requires that both the signature and \(\Delta^\I\) are finite (which is reasonable for normalized \ELH), otherwise the vectors in \(\geointerp\) would have infinite dimension.
%and the extension of each concept might have infinitely many elements. 
